Facets for Art Gallery Problems

The Art Gallery Problem (AGP) asks for placing a minimum number of stationary guards in a polygonal region P, such that all points in P are guarded. The problem is known to be NP-hard, and its inherent continuous structure (with both the set of points that need to be guarded and the set of points that can be used for guarding being uncountably infinite) makes it difficult to apply a straightforward formulation as an Integer Linear Program. We use an iterative primal-dual relaxation approach for solving AGP instances to optimality. At each stage, a pair of LP relaxations for a finite candidate subset of primal covering and dual packing constraints and variables is considered; these correspond to possible guard positions and points that are to be guarded. Particularly useful are cutting planes for eliminating fractional solutions. We identify two classes of facets, based on Edge Cover and Set Cover (SC) inequalities. Solving the separation problem for the latter is NP-complete, but exploiting the underlying geometric structure, we show that large subclasses of fractional SC solutions cannot occur for the AGP. This allows us to separate the relevant subset of facets in polynomial time. We also characterize all facets for finite AGP relaxations with coefficients in {0, 1, 2}. Finally, we demonstrate the practical usefulness of our approach. Our cutting plane technique yields a significant improvement in terms of speed and solution quality due to considerably reduced integrality gaps as compared to the approach by Kr\"oller et al.

==> definitions.tex <==
\section{Notations and Preliminaries}\label{sec:not}

We consider a polygonal region $P$ with $n$ vertices that may have holes, \ie, that does not have to be simply connected.
For a point $p\in P$, we denote by $\V(p)$ the {\em visibility polygon} of $p$ in $P$, \ie, the set of
all $q\in P$, such that the straight-line connection $\overline{p,q}$ lies completely in $P$; by definition, $\V(p)$ is star-shaped.
For a set $S\subseteq P$, $\V(S):=\cup_{p\in S} \V(p)$.
A set $C\subseteq P$ is a {\em guard cover}, if $\V(C)=P$.
The {\em Art Gallery Problem} asks for a guard cover
of minimum cardinality; this is the same as covering $P$ by a minimum number of star-shaped sub-regions of $P$.

For simplicity, we abbreviate $x(G) := \sum_{g \in G} x_g$ for any vector $x$.

